MedCodER: A Generative AI Assistant for Medical Coding

Medical coding is essential for standardizing clinical data and communication but is often time-consuming and prone to errors. Traditional Natural Language Processing (NLP) methods struggle with automating coding due to the large label space, lengthy text inputs, and the absence of supporting evidence annotations that justify code selection. Recent advancements in Generative Artificial Intelligence (AI) offer promising solutions to these challenges. In this work, we introduce MedCodER, a Generative AI framework for automatic medical coding that leverages extraction, retrieval, and re-ranking techniques as core components. MedCodER achieves a micro-F1 score of 0.60 on International Classification of Diseases (ICD) code prediction, significantly outperforming state-of-the-art methods. Additionally, we present a new dataset containing medical records annotated with disease diagnoses, ICD codes, and supporting evidence texts (https://doi.org/10.5281/zenodo.13308316). Ablation tests confirm that MedCodER's performance depends on the integration of each of its aforementioned components, as performance declines when these components are evaluated in isolation.

==> dep.tex <==
% Original Our Work + Baselines
\section{Methods}
% Moved Dataset to its own section
\subsection{Our Work}
\label{novelty}
Our aim is quite different from methods previously described in literature. A primary line of previous research work focuses on the identification of diseases, and another disparate line of work is on the automated identification of ICD codes. However, our objectives are three pronged:

\begin{enumerate}

    \item Identification of diseases diagnosed in the patient: It is important to note that although many disease may be mentioned in the medical note, only the final diagnosed ones are important for medical coding purposes. Also, symptoms for diseases for e.g. "chest pain" in "myocardial infarction", should not be included as diagnoses.
    
    \item Identification of evidence or support sentences: These are the supporting sentences, maybe containing signs and symptoms, treatment plan, medications etc. for a specific diagnosis. These sentences serve as evidence which reinforce the diagnosis.
    
    \item Identification of the ICD codes: For every identified disease diagnosis, the corresponding specific / valid ICD codes are also identified.
    
\end{enumerate}
By working towards these objectives, the final goal is to develop a software assistant which can aid trained medical coders to carry out their ICD coding tasks with increased efficiency and / or accuracy.

% Put this in experiments section?
\subsection{Baseline Approaches}
We considered multiple baseline approaches described in literature. However, one major distinction in the previously described approaches is that their objectives are only focused on one task - either disease entity recognition \textbf{REFERENCE} or ICD prediction \textbf{REFERENCE}. Here are the baseline methods we considered:
\begin{itemize}
    \item \textbf{Disease Diagnosis Identification}: Although there is no method described in literature that focuses specifically on identifying diagnosed diseases, there are many which focus on biomedical named entity (including disease) recognition. Multiple named entity recognition (NER) methods able to identify diseases have been described in literature \textbf{REFERENCE}. We use as baseline  GliNER \textbf{REFERENCE}, one of the best performing zero-shot NER method. It is important to note that these NER methods are not focused on disease diagnosis detection. Therefore, they would identify all disease mentions in the text, irrespective of whether that is the diagnosed disease or not, leading to many false positives.
    \item \textbf{Supporting Evidence Identification}: To the best of our knowledge, no supporting evidence identification method has been described in literature.
    \item \textbf{ICD Code Prediction}: Many methods for ICD Code prediction has been described in literature, some of them have been mentioned in Section \ref{related_work}. We focused on the following as baselines:
    \begin{enumerate}
        \item PLM-ICD \textbf{REFERENCE}: This method focuses on a training a pretrained masked language model on labelled ICD datasets. Since our dataset was too small to train such a model, we used the pretrained model weights from \textbf{REFERENCE} for inference on our dataset.
        \item TreeLLM \textbf{REFERENCE}: This is a generative AI based method which sequentially traverses the ICD Code Hierarchy and finds the most relevant ICD Codes for a given medical note.
    \end{enumerate}
    
    \item 
\end{itemize}

\section{Dataset}
Although many datasets for medical record coding have been described in literature, they suffer from two major problems, particularly with respect to the problem being addressed in this work:
\begin{enumerate}
    \item Focus on one task: Majority of the medical record datasets focus only on the identification of ICD codes \textbf{REFERENCE}. However, our methodologies of identifying disease diagnosis and supporting evidence could not be developed and evaluated using these datasets.
    \item Restrictive commercial licensing: Due to several reasons including but not limited to patient confidentiality and commercial reasons, majority of the publicly available datasets are not open for commercial use.
\end{enumerate}
Due to the above reasons, a new dataset was built using publicly available open source datasets. Since most real medical record datasets have very restrictive licenses in order to maintain privacy, we focused on a synthetic dataset. ACI-Bench [\textbf{REFERENCE}] was first introduced as a medical conversation summarization dataset where the objective was to convert a conversation between a patient and a caregiver to a summarized medical or clinical note. Both the conversation and the summaries provided were synthetic, and hence devoid of the usage restrictions typically associated with real world medical records. 

Here is the brief process for creation of the dataset:
\begin{enumerate}
    \item The ACI Bench summarized clinical notes were extracted and cleaned.
    \item The individual clinical notes were uploaded to TeamTat \textbf{REFERENCE}, a tool commonly used for annotating biomedical information extraction datasets.
    \item Expert medical coders with decades of experience and practice in the field annotated the dataset.
\end{enumerate}


The following details were annotated by the experts:

\begin{enumerate}
    \item Disease Diagnosis terms / phrases.
    \item Evidence sentences.
    \item ICD Code for the diagnosis.
\end{enumerate}

Here are the overall dataset statistics:
\textbf{DATASET STATS TABLE GOES HERE \\
SPLIT BY TRAIN/TEST/VAL \\
1. Number of datapoints. \\
2. Number of unique ICD Codes. \\
3. Number of diagnoses. \\
4. Number of evidence sentences. \\
FEEL FREE TO ADD MORE
}



\section{Proposed Framework}
The goal of our proposed framework is to show how LLMs can be used to develop an interpretable ICD coding methodology and increase the efficiency of medical coders. Not only does our framework suggest relevant ICD-10 codes for a medical record, it also In addition to producing ICD codes, our framework also has the capability to produce increase the efficiency of medical coders by providing them with ICD code recommendations and relevant medical record texts. To do this, we expand on the traditional automatic ICD coding objective by adding diagnosis and supporting evidence extraction. This allows us to augment our coding methodology with more relevant information and provide insight into the medical record even when ICD code predictions are incorrect.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{focused_l1.png}
    \caption{High level Schematic Diagram of the Methodology}
    \label{fig:detailed}
\end{figure*}

% INSERT METHODOLOGY FIGURE HERE.

A schematic diagram containing the methodology is depicted in figure \ref{fig:detailed}.

\begin{figure}[htbp]
    \centering
    \includesvg{our_prompt_1.svg}
    \caption{High level Schematic Diagram of the Methodology}
    \label{fig:prompt}
\end{figure}

\subsubsection{Diagnosis, Supporting Evidence \& ICD Code Extraction}
The first step of the process involves using an LLM viz. GPT-4 to identify all the diagnosed diseases, along with their supporting evidence and corresponding ICD Code. It is important to note that in this step, the inherent knowledge of the LLM is used to extract the diagnosis, supporting evidence and ICD Codes. The actual prompt can be found in Figure \ref{fig:main}. It is important to note that there is a possibility for the LLM to hallucinate and produce incorrect predictions. In order to counter this, we do the following:

\begin{enumerate}
    \item \textbf{Finding Diagnosis Mention}: The text segment most similar to the diagnosis predicted by the LLM is extracted using fuzzysearch, and their locations are predicted as the final diagnosis mentions.
    \item \textbf{Finding Supporting Evidence Sentences}: The sentences with the highest similarity using BM25 [REFERENCE] with the predicted "Supporting Evidence" sentences are found and their start and end locations are predicted as the supporting evidence.
    \item \textbf{Augmenting ICD Codes}: The ICD Codes are further augmented using retrieval and reranking, the process is detailed in the subsequent sections.
\end{enumerate}

\subsubsection{ICD Retrieval Augmentation}
The diagnosed disease is used to identify candidate ICD codes. Briefly, as a preprocessing step, a vector database collection is created using the ICD codes and their descriptions, where the descriptions are converted into embeddings using the OpenAI Ada 2 model [REFERENCE]. During inference, for every disease diagnosis identified in the prompting step, an embedding vector is created using the same Ada2 model, and this embedding is used to search and retrieve the most similar ICD Code descriptions. This produces a ranked list of ICD codes which are similar to the diagnosed disease.

\subsubsection{Code-to-Record Re-ranking}
The candidate retrieved ICD Codes, along with the ICD code produced by prompting are further reranked using RankGPT, a methodology for reranking using LLM prompting [REFERENCE]. For the reranking step, the LLM is provided additional details which were left out for the retrieval step, viz. the supporting evidence, as often, the final ICD code for a particular condition depends on a variety of additional context about the disease, apart from the diagnosed disease name.


\section{Experiments}
TODO: Make this shorter
\subsection{Metrics Used for Evaluation}
As mentioned in the previous section, the our methodology has multiple components, and these components are evaluated in isolation. 

\subsubsection{Disease Diagnosis Extraction}

The disease diagnosis extraction can be evaluated by posing it as an entity extraction or named entity recognition task. There are two methods that can be used for evaluation.

\begin{enumerate}
    \item The first method for evaluating Disease Diagnosis Extraction is based on sequence (of words) labelling, which takes into account partial matches between predicted and ground truth spans of recognised entities. The metrics are \textbf{Exact Match} and \textbf{Partial Match}. Detailed description of the evaluation methodology can be found in \cite{semeval9.1, muc, semeval_blog}. 
    \item The second method is a more straight forward. It compares the set of texts extracted by the methods as disease diagnosis with the ground truth ones, using precision, recall and F1 to indicate the performance. [ELIJAH ADD REASONING]
\end{enumerate}

\subsubsection{Supporting Evidence Extraction}
The supporting evidence extraction can also be evaluated by posing it as an span extraction task. We compare the predicted supporting evidence sentences extracted by the methodology with the ground truth, and quantify the performance using \textbf{Exact Match} and \textbf{Partial Match} metrics described above \cite{semeval9.1, muc, semeval_blog}.

\subsubsection{ICD Code Prediction}
For evaluating the performance of ICD code prediction component, we used traditional precision, recall and F1, where we compare the set of predicted ICDs with the set of ground truth ICDs.

It is important to note that our method is unlike most methods which found in literature, and poses the ICD code prediction problem somewhat like an information retrieval task. Therefore, for each of the disease diagnosis extracted from a medical record, a ranked list of ICD Codes would be predicted. For comparison with baselines, the cutoff (or K) value is taken as 1. However, in order to ensure that the correct code for a particular diagnosis is present in the predicted set, a higher value of K can also be used. As we increase the cutoff (or K), the recall of the methodology would increase, however at the cost of lower precision. In order to quantify the trade-off, the precision, recall and F1 scores at different values of K viz. 1, 2, 5, 10 and 20 are used.


We considered multiple baseline approaches described in literature. However, one major distinction in the previously described approaches is that their objectives are only focused on one task - either disease entity recognition \textbf{REFERENCE} or ICD prediction \textbf{REFERENCE}. Here are the baseline methods we considered:
\begin{itemize}
    \item \textbf{Disease Diagnosis Identification}: Although there is no method described in literature that focuses specifically on identifying diagnosed diseases, there are many which focus on biomedical named entity (including disease) recognition. Multiple named entity recognition (NER) methods able to identify diseases have been described in literature \textbf{REFERENCE}. We use as baseline  GliNER \textbf{REFERENCE}, one of the best performing zero-shot NER method. It is important to note that these NER methods are not focused on disease diagnosis detection. Therefore, they would identify all disease mentions in the text, irrespective of whether that is the diagnosed disease or not, leading to many false positives.
    \item \textbf{Supporting Evidence Identification}: To the best of our knowledge, no supporting evidence identification method has been described in literature.
    \item \textbf{ICD Code Prediction}: Many methods for ICD Code prediction has been described in literature, some of them have been mentioned in Section \ref{related_work}. We focused on the following as baselines:
    \begin{enumerate}
        \item PLM-ICD \textbf{REFERENCE}: This method focuses on a training a pretrained masked language model on labelled ICD datasets. Since our dataset was too small to train such a model, we used the pretrained model weights from \textbf{REFERENCE} for inference on our dataset.
        \item TreeLLM \textbf{REFERENCE}: This is a generative AI based method which sequentially traverses the ICD Code Hierarchy and finds the most relevant ICD Codes for a given medical note.
    \end{enumerate}
    
    \item 
\end{itemize}

\subsection{Ablation Studies}

In order to evaluate the efficacy of the different choices of architecture followed in our methodology, we carry out extensive ablation studies.

\subsubsection{Performance Gain Due to Retrieval and Reranking}

As shown in the results (Section\ref{results}), LLMs like GPT4 inherently contains knowledge about ICD Coding, as indicated with the decent performance of direct prompting based methods for ICD coding. In order to evaluate the value added by the retriever and the reranker in ICD Coding, we quantify the precision, recall and F1 at different values of K.

\subsection{Experiment with Users}
In order to evaluate the gain in efficiency and accuracy of coders using the tool, we carry out an controlled study. In this,. The codes provided by them were noted, along with the time taken for them to code each record.
